General Detection-based Text Line Recognition

We introduce a general detection-based approach to text line recognition, be it printed (OCR) or handwritten (HTR), with Latin, Chinese, or ciphered characters. Detection-based approaches have until now been largely discarded for HTR because reading characters separately is often challenging, and character-level annotation is difficult and expensive. We overcome these challenges thanks to three main insights: (i) synthetic pre-training with sufficiently diverse data enables learning reasonable character localization for any script; (ii) modern transformer-based detectors can jointly detect a large number of instances, and, if trained with an adequate masking strategy, leverage consistency between the different detections; (iii) once a pre-trained detection model with approximate character localization is available, it is possible to fine-tune it with line-level annotation on real data, even with a different alphabet. Our approach, dubbed DTLR, builds on a completely different paradigm than state-of-the-art HTR methods, which rely on autoregressive decoding, predicting character values one by one, while we treat a complete line in parallel. Remarkably, we demonstrate good performance on a large range of scripts, usually tackled with specialized approaches. In particular, we improve state-of-the-art performances for Chinese script recognition on the CASIA v2 dataset, and for cipher recognition on the Borg and Copiale datasets. Our code and models are available at https://github.com/raphael-baena/DTLR.

==> dump.tex <==
        % \begin{minipage}{0.33\linewidth}
        %         \centering
        %         \includegraphics[width=\linewidth]{Figures/HWDB_pretty_plots_ranked_worst_3/3236.png}
        %         \vspace{0.4em}
        %         \parbox{\linewidth}{
        %             \centering 
        %             \scriptsize 
        %             \texttt{P: } \begin{CJK*}{UTF8}{gbsn} 冬瓜、黄瓜、西瓜、西红柿、绿豆、绿豆芽、黄豆芽、豆腐、莲藕、椹、柚\end{CJK*}\\[-0.2em]
        %             \texttt{GT: } \begin{CJK*}{UTF8}{gbsn} 冬瓜, 黄瓜, 西瓜, 西红柿, 绿豆、绿豆芽, 黄豆芽, 豆腐, 莲藕梨, 桑椹, 柚\end{CJK*}\\[-0.2em]
        %         }
                
        %     \end{minipage} & 
        % \begin{minipage}{0.33\linewidth}
        %         \centering
        %         \includegraphics[width=\linewidth]{Figures/HWDB_pretty_plots_ranked_worst_3/7968.png}
        %         \vspace{0.4em}
        %         \parbox{\linewidth}{
        %             \centering 
        %             \scriptsize 
        %             \texttt{P: }  \begin{CJK*}{UTF8}{gbsn}1  8  法国传任住与在花重部首次年到崖座柏本, 此后的\end{CJK*}\\[-0.2em]
        %             \texttt{GT: }  \begin{CJK*}{UTF8}{gbsn}1 8 9 2 年法国传士在重庆市首次采集到崖柏标本。此后1 0 0 \end{CJK*}
        %         }
        %     \end{minipage} & 
        % \begin{minipage}{0.33\linewidth}
        %         \centering
        %         \includegraphics[width=\linewidth]{Figures/HWDB_pretty_plots_ranked_worst_3/7970.png}
        %         \vspace{0.4em}
        %         \parbox{\linewidth}{
        %             \centering 
        %             \scriptsize 
        %             \texttt{P: }  \begin{CJK*}{UTF8}{gbsn}和字巴也再再新的的况。 年前, 也世界保护比比地们\end{CJK*}\\[-0.2em]
        %             \texttt{GT: }  \begin{CJK*}{UTF8}{gbsn}和文字也再新的的况录。9 年前, 世界保护联盟( I U C N  \end{CJK*}
        %         }
        %     \end{minipage} \\





        %CIPHER
        \begin{minipage}{0.33\linewidth}
            \centering
            \includegraphics[width=\linewidth]{Figures/Copiale_worst/Copiale_0.png}
            \vspace{0.4em}
                \parbox{\linewidth}{\centering \scriptsize \texttt{P:} $z \dot{r}  \gamma c. \underline{m} : \underline{u} o \ddot{y}  \underline{r} b \dot{x}  z | \hat{a} c.: \dagger  \dot{n}  \hat{\iota}  : \lambda c \hat{\iota}  j\hat{i}+z \hat{a} js \gamma  \hat{o}  \eta  \underline{n} \hat{i}p \dot{s}  \hat{a}  \iota bas \saturn  \underline{u} s \delta  \mathit{g}  \pluto  \underline{u} a| \Lambda c. \iota  \underline{m} bas \gamma i|g \dot{n}  
eq  \dot{x}  \hat{o} r.$}
            \parbox{\linewidth}{\centering \scriptsize \texttt{GT: }$ \hat{o}  \dot{r}  \gamma \hat{i} \underline{m} : \underline{u} o \ddot{y}  \underline{r} b \dot{x}  z | \hat{a} c.: \dagger  \dot{n}  \hat{\iota}  : \lambda c \hat{\iota}  j\hat{i}+z \hat{a} js \gamma  \hat{o}  \eta  \underline{n} \hat{i}p \dot{s}  \hat{a}  \iota bas \saturn  \underline{u} s \delta  \mathit{g}  \pluto  \underline{u} a$}
        \end{minipage} & 
        \begin{minipage}{0.33\linewidth}
            \centering
            \includegraphics[width=\linewidth]{Figures/Copiale_worst/Copiale_1.png}
            \vspace{0.4em}
            \parbox{\linewidth}{\centering \scriptsize \texttt{P:} $ z \mathit{g} 3kp \Lambda oi \hat{u} jg \pluto  \hat{\iota}  p. \saturn c.Zz \hat{e} +g3 \pluto  \hat{\iota}   \mathit{g} 3p.= \hat{\iota}  | z  \saturn  \hat{a} 3u+ \eta  \sagittarius  \delta c.3Xr \dot{s} = \delta $}
            \parbox{\linewidth}{\centering \scriptsize \texttt{GT:} $z \mathit{g} 3kp \Lambda oi \hat{u} jg \pluto \hat{i} \hat{\iota}  p. \saturn c.Zz \hat{e} + \female c. \lambda \hat{i}hk \underline{u} g3 \pluto  \mathit{g} 3p.= \hat{\iota}  | z  \saturn  \hat{a} 3u+ \eta  \sagittarius \delta c.3Xr \dot{s} =\delta$}
        \end{minipage} & 
        \begin{minipage}{0.33\linewidth}
            \centering
            \includegraphics[width=\linewidth]{Figures/Copiale_worst/Copiale_2.png}
            \vspace{0.4em}
            \parbox{\linewidth}{\centering \scriptsize \texttt{P:} $v \lambda \hat{i}+d: \hat{o} c. \pluto h.=o \male 3+k \lambda o. \pi \hat{i}rz \hat{u} |m \saturn  \iota 3 \dot{n} +|vo \gamma grlX \lambda f=gz$}
            \parbox{\linewidth}{\centering \scriptsize \texttt{GT: } $v \lambda \hat{i}+d: \hat{o} c. \pluto h.=o \male 3+k \lambda o. \pi \hat{i}rz \hat{u} hn \saturn  \iota 3 \dot{n} +|vlongslongso \gamma grlX \lambda f=gz$}
        \end{minipage} \\




                \begin{minipage}{0.33\linewidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/IAM_pretty_plots_ranked_worst_3/2654.png}
                \vspace{0.4em}
                \parbox{\linewidth}{
                    \centering 
                    \scriptsize 
                    \texttt{P: wen ence au ase}\\[-0.2em]
                    \texttt{GT: -----------------------------------------------------}
                }
            \end{minipage} & 
            \begin{minipage}{0.33\linewidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/IAM_pretty_plots_ranked_worst_3/2741.png}
                \vspace{0.4em}
                \parbox{\linewidth}{
                    \centering 
                    \scriptsize 
                    \texttt{P: " Buls You! 1 toPE LukE is suitrsus cenrml, emouin. " ' Olt, won,, '}\\[-0.2em]
                    \texttt{GT:  " Bless you! I hope Luke is suitably grateful, darling. " " Oh, well, "}
                }
            \end{minipage} & 
            \begin{minipage}{0.33\linewidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/IAM_pretty_plots_ranked_worst_3/2742.png}
                \vspace{0.4em}
                \parbox{\linewidth}{
                    \centering 
                    \scriptsize 
                    \texttt{P: HE StouCG DifFIDENTU, ' I Li ETH Nook. oNE GES paNts}\\[-0.2em]
                    \texttt{GT: he shrugged diffidently, " I like the work. One gets plenty}
                }
            \end{minipage} \\
            \begin{minipage}{0.33\linewidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/RIMES_pretty_plots_ranked_worst_3/246.png}
                \vspace{0.4em}
                \parbox{\linewidth}{
                    \centering 
                    \scriptsize 
                    \texttt{P: N° Dubois. Je souhaiterais étre  cavut as titre de la raponsabilité}\\[-0.2em]
                    \texttt{GT: Md Dubois je souhaiterais être couvert au titre de la responsabilité}
                }
            \end{minipage} & 
            \begin{minipage}{0.33\linewidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/RIMES_pretty_plots_ranked_worst_3/661.png}
                \vspace{0.4em}
                \parbox{\linewidth}{
                    \centering 
                    \scriptsize 
                    \texttt{P: peerrendls, j'aiétédans l'obligation de léturer mon compte (N° 003703A80165)}\\[-0.2em]
                    \texttt{GT: personnelles, j'ai été dans l'obligation de clôturer mon compte (N° 90370DA80165)}
                }
            \end{minipage} & 
            \begin{minipage}{0.33\linewidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/RIMES_pretty_plots_ranked_worst_3/764.png}
                \vspace{0.4em}
                \parbox{\linewidth}{
                    \centering 
                    \scriptsize 
                    \texttt{P: Ca lêture ne pradpas eflet immmédiatennt, mais à compter du 01/03/r00s.}\\[-0.2em]
                    \texttt{GT: La clôture ne prend pas effet immédiatement, mais à compter du 01/03/2007.}
                }
            \end{minipage}\\

